Runtime Verification Through Forward Chaining

In this paper we present a novel rule-based approach for Runtime Verification of FLTL properties over finite but expanding traces. Our system exploits Horn clauses in implication form and relies on a forward chaining-based monitoring algorithm. This approach avoids the branching structure and exponential complexity typical of tableaux-based formulations, creating monitors with a single state and a fixed number of rules. This allows for a fast and scalable tool for Runtime Verification: we present the technical details together with a working implementation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{68}
\providecommand{\publicationstatus}{Nikolaj Bj{\o}rner, Fabio Fioravanti, Andrey Rybalchenko, \\ Valerio Senni (Eds.): First Workshop on \\ Horn Clauses for Verification and Synthesis (HCVS 2014)\\
EPTCS 169, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.169.8}{10.4204/EPTCS.169.8}}
\pdfoutput=1

